A radio, optical, UV and X-ray view of the enigmatic changing look Active Galactic Nucleus 1ES~1927+654 from its pre- to post-flare states

The nearby type-II AGN 1ES1927+654 went through a violent changing-look (CL) event beginning December 2017 during which the optical and UV fluxes increased by four magnitudes over a few months, and broad emission lines newly appeared in the optical/UV. By July 2018 the X-ray coronal emission had completely vanished, only to reappear a few months later. In this work we report the evolution of the radio, optical, UV and X-rays from the pre-flare state through mid-2021 with new and archival data from the Very Long Baseline Array (VLBA), the European VLBI Network, the Very Large Array (VLA), the Telescopio Nazionale Galileo (TNG), Gran Telescopio Canarias (GTC), The Neil Gehrels Swift observatory and XMM-Newton. The main results from our work are: (1) The source has returned to its pre-CL state in optical, UV, and X-ray; the disk-corona relation has been re-established as has been in the pre-CL state, with an $\alpha_{\rm OX}\sim 1.02$. The optical spectra are dominated by narrow emission lines. (2) The UV light curve follows a shallower slope of $\propto t^{-0.91\pm 0.04}$ compared to that predicted by a tidal disruption event. We conjecture that a magnetic flux inversion event is the possible cause for this enigmatic event. (3) The compact radio emission which we tracked in the pre-CL (2014), during CL (2018) and post-CL(2021) at spatial scales $<1$ pc was at its lowest level during the changing look event in 2018, nearly contemporaneous with a low $2-10$ keV emission. The radio to X-ray ratio of the compact source $L_{\rm Radio}/L_{\rm X-ray}\sim 10^{-5.5}$, follows the Gudel-Benz relation, typically found in coronally active stars, and several AGN. (4) We do not detect any presence of nascent jets at the spatial scales of $\sim 5-10$ pc.

==> tab_specfeat_postCL.tex <==
\begin{table*}
    \begin{center}
    \caption{The post-changing-look optical spectral features observed by GTC/OSIRIS in 2021  \label{tab:gtc_lines}}
    \begin{tabular}{lcccc}
       \hline
       \hline
       Line ID  & Center & FWHM & Line Flux & Comment$\rm ^B$  \\ 
     &   (\AA)  & ($\rm km\,s^{-1}$) & ($\funit{}$)  \\
     &    &  & $\times 10^{-15}$  \\
     
        \hline
$\rm [OII]3727$ & $3796.8 \pm 0.6$ & $710/285 \pm 100$ &  $2.34 \pm 0.4$ & new line  \\
$\rm HeII4686$ & $4775.1 \pm 0.4$  & $795/603 \pm 80$  &  $0.99 \pm 0.11$ & new line \\
$\rm H\beta$ & $4953.3 \pm 0.4$ & $660/435 \pm 30$ &  $1.43 \pm 0.08$  &same \\
$\rm [OIII]4959$ & $5052.09 \pm 0.03$ & $505/125 \pm 4$ & $1.95 \pm 0.02$ &lower ($-15\%$) \\
$\rm [OIII]5007$ & $5100.92 \pm 0.03$  & $505/143 \pm 4$ &  $5.91 \pm 0.06$ & lower ($-13\%$) \\
$\rm [OI]6300$ & $6417.56 \pm 0.82$ & $477/281 \pm 86$ & $0.29 \pm 0.07$ & new line\\
$\rm [NII]6548$ & $6670.00 \pm 0.19$ & $500/335 \pm 22$ &  $0.66 \pm 0.04$ & higher ($+22\%$)  \\
$\rm H\alpha$ & $6686.22 \pm 0.08$  & $544/400 \pm 9$ &  $5.64 \pm 0.13$  &higher ($+18\%$) \\
$\rm [NII]6584$ & $6706.06 \pm 0.20$ & $500/352 \pm 22$ &  $2.00 \pm 0.11$  &higher ($+22\%$) \\
        \hline 
        \hline
\end{tabular}
    
\end{center}

\tablecomments{ The post-changing-look optical spectral features measured from the combined spectrum after stellar template subtraction.  The spectrum has been corrected for Galactic extinction. 
    %Notes: $^a$ Due to the stellar absorption, H${\beta}$ is detected in absorption in the observed spectrum and in emission after the stellar correction.
The center and width of the lines [OIII]~4959,5007\Angstrom\Angstrom\ and [N~II]~6548,6584\Angstrom\Angstrom\ are tied. The line flux ratios [OIII]~5007/4959 and [N~II]~6584/6548 are kept fixed to the theoretical value 3. \\
{$\rm ^B$ Listing the instances when the lines in the post-CL (2021) spectra have lower, higher or similar fluxes compared to the pre-CL spectra (2011) reported in Table \ref{Table:dolores_lines}}. }
The two line width values correspond to  the measured/deconvolved by the instrumental line profile. 
    

\end{table*}

%$\rm{[O~II] 3727}$ &  3796.8$\pm$0.6 & 710$\pm$90 & 2.34$\pm$0.40 & 2.9$\pm$1.2 \\
%$\rm{He~II 4686}$ &  4775.1$\pm$0.4 &  795$\pm$70 & 0.99$\pm$0.11 & 1.5$\pm$0.2 \\
%H${\beta}^a$  & 4953.3$\pm$0.2 & 647$\pm$25 & 1.38$\pm$0.08 & -3.7$\pm$0.3 \\
%$\rm{[O~III] 4959}$ & 5051.99$\pm$0.09 & 492$\pm$9 & 1.84$\pm$0.05 & 3.98$\pm$0.19 \\
%$\rm{[O~III] 5007}$ & 5100.95$\pm$0.03 & 506$\pm$4 & 5.96$\pm$0.06 & 10.7$\pm$0.2 \\
%$\rm{[O~I] 6300}$   & 6417.6$\pm$0.8 & 477$\pm$84 & 0.29$\pm$0.06 & 1.1$\pm$0.3 \\
%$\rm{[N~II] 6548}^b$ & 6670.7$\pm$0.5 & 361$\pm$52 & 0.49$\pm$0.09  & 1.19$\pm$0.16 \\
%H${\alpha}^b$  & 6686.15$\pm$0.08 & 545$\pm$10 & 5.63$\pm$0.13  & 13.4$\pm$0.2 \\
%$\rm{[N~II] 6584}^b$   & 6706.0$\pm$0.2 & 505$\pm$24 & 2.01$\pm$0.18  & 5.0$\pm$0.2 \\


==> tab_specfeat_preCL.tex <==
\begin{table*}
    \begin{center}
        
    \caption{Pre-changing-look optical spectral features, observed in 2011 by TNG\label{Table:dolores_lines}}

    \begin{tabular}{lccc}
       \hline
       \hline
   
Line & wavelength & FWHM & Line Flux \\ 
     & ($\angs$) & ($\kms$) &  ($\funit{}$)\\
     &  &  &   ($ \times 10^{-15}$)\\
\hline

%$\rm HeII4686$ & $4775.0 \pm 0.9$ & & $405.8 \pm 140$ &  $0.56 \pm 0.2$  \\
$\rm H\beta$ & $4952.1 \pm 0.7$ &  $555/310 \pm 135$  &  $1.25 \pm 0.37$ \\
$\rm [OIII]4959$ & $5052.45 \pm 0.11$ &  $521/261 \pm 14$  & $2.25 \pm 0.08$ \\
$\rm [OIII]5007$ & $5101.29 \pm 0.11$  &  $521/268 \pm 14$ & $6.81 \pm 0.24$ \\
$\rm [NII]6548$ & $6668.4 \pm 1.0$ &  $417/240 \pm 140$ & $0.51 \pm 0.18$ \\
$\rm H\alpha$\tablenotemark{\footnotesize A} & $6682.6 \pm 0.51$ &  $721/636 \pm 70$  & $4.09 \pm 0.43$\\
$\rm [NII]6584$ & $6704.4 \pm 1.0$ &  $417/242 \pm 140$ & $1.55 \pm 0.53$ \\
\hline\\
\end{tabular}

\hspace{1.5cm}{H$\alpha$ profile modelled by a broad and a narrow component.}\\
\\

\begin{tabular}{lccc}
\hline 
$\rm [NII]6548$ & $6668.0 \pm 0.5$  &  $421/247 \pm 14$ & $0.43 \pm 0.07$  \\
$\rm H\alpha-n$\tablenotemark{\footnotesize B} & $6683.0 \pm 0.5$ &  $625/524 \pm 60$ & $3.13 \pm 0.49$  \\
$\rm H\alpha-b$\tablenotemark{\footnotesize B} & $6673.18 \pm 15$ & $2644/2621 \pm 700$ & $2.10 \pm 1.25$  \\
$\rm [NII]6584$ & $6704.49 \pm 0.69$ & $421/249 \pm 85.3$ & $1.29 \pm 0.22$  \\

        \hline 
        \hline
    \end{tabular}
    \end{center}

\tablenotetext{\footnotesize A}{With a single Gaussian line fit to the H$\alpha$ complex we found that the line is slightly broad.}
  
\tablenotetext{\footnotesize B}{The H$\alpha$ emission line was modelled using two Gaussian components for H$\alpha$: narrow H$\rm \alpha-n$ and broad H$\rm \alpha-b$. In this case, the line width of [NII]$6548, 6584$ were fixed to the value obtained with a single component.}  

\tablecomments{Measurements of the spectral features in the pre-changing-look optical spectrum, observed in 2011 by TNG/LRB. The spectrum has been corrected for Galactic extinction. The host galaxy stellar emission has been subtracted.  The two line width values correspond to the measured/deconvolved by the instrumental profile. The complex H$\alpha+[NII]$ has been fitted in two modes: first using a single component for each spectral feature, and second using two components for H$\alpha$, quoted below the horizontal line. In the second mode the line width for [NII]$6548, 6584$ were kept fixed to the value obtained in the first case.}    
    
\end{table*}

